Weakly Supervised AUC Optimization: A Unified Partial AUC Approach

Since acquiring perfect supervision is usually difficult, real-world machine learning tasks often confront inaccurate, incomplete, or inexact supervision, collectively referred to as weak supervision. In this work, we present WSAUC, a unified framework for weakly supervised AUC optimization problems, which covers noisy label learning, positive-unlabeled learning, multi-instance learning, and semi-supervised learning scenarios. Within the WSAUC framework, we first frame the AUC optimization problems in various weakly supervised scenarios as a common formulation of minimizing the AUC risk on contaminated sets, and demonstrate that the empirical risk minimization problems are consistent with the true AUC. Then, we introduce a new type of partial AUC, specifically, the reversed partial AUC (rpAUC), which serves as a robust training objective for AUC maximization in the presence of contaminated labels. WSAUC offers a universal solution for AUC optimization in various weakly supervised scenarios by maximizing the empirical rpAUC. Theoretical and experimental results under multiple settings support the effectiveness of WSAUC on a range of weakly supervised AUC optimization tasks.

==> tabcmd_text.tex <==
% Cell alignment command for mean +/- std (text version).
% 
% Author: Zheng Xie
% Date: 2024.01.07
% 
% This file provides an alternative (and sometimes better) way for producing 
% aligned column of mean +/- std, than using siunitx package.
% 
% By calling:
%     \msc{90.12}         (for mean only), or 
%     \msc{90.12,}        (for mean only, but align with cells with std's), or 
%     \msc{90.12,3.45}    (for mean +/- std),
% the column will be aligned at the separator, the decimal point of the mean (if
% all means have the same digits after decimal point), and the decimal point of 
% the std (if all std's have the same digits before decimal point). The overall 
% column can be aligned left/right/centered according to the tabular options. 
% The numbers will be in math font, the std will be printed as subscripts.
% To bold the cell, just call:
%     \msc[b]{90.12,3.45} 
% or simply
%     \msb{90.12,3.45}   
% A key advantage of this command is that the bold font is implemented to be of 
% the same width of normal numbers, so that making cells bold does not affect
% alignment.
% 
% You can use the command:
%     \setcellformat[std alignment]{mean format}{sep}{std format}
% at the beginning of the table to setup the command.
% example:
%     \setcellformat[l/r]{00.00}{\ensuremath{_\pm}}{00.00}
% the default setting is:
%     \setcellformat[l]{00.00}{\ensuremath{_\pm}}{00.00}
% If you want to use the mean only, its recommended to set the last two options
% empty so that the numbers are not shifted to the left.
% 
% The mean/std format determines the space the number will taken. Making std 
% align to the left is the default option, which usually make the numbers close 
% to the separator but not aligned at their decimal points if they have 
% different magnitudes. 
% 
% Other examples:
% Highlighting the percentage of increment:
%     \renewcommand{\basicstdstyle}[1]{{\color{red} +#1\%}}
%     \setcellformat[l]{00.00}{}{00.00}
% Put the std in parentheses:
%     \renewcommand{\basicstdstyle}[1]{(#1)}
%     \setcellformat[l]{00.00}{}{00.00}

\usepackage{listofitems}
\usepackage{mathtools}

\newcommand\msmfmt{00.00}
\newcommand\mssep{\ensuremath{_\pm}}
\newcommand\mssfmt{\textsubscript{00.00}}
\newcommand\msstdalign{l}

\newcommand{\basicmeanstyle}[1]{#1}%
\newcommand{\basicstdstyle}[1]{#1}%
\newcommand*\bfmeanstyle[1]{\textbf{\basicmeanstyle{#1}}}%
\newcommand*\bfstdstyle[1]{\textbf{\basicstdstyle{#1}}}%

\newlength{\meanlen}
\newlength{\stdlen}
\settowidth{\meanlen}{{\basicmeanstyle{\msmfmt}}}
\settowidth{\stdlen}{{\basicstdstyle{\mssfmt}}}

\newcommand{\meanstyle}[1]{\basicstdstyle{#1}}%
\newcommand{\stdstyle}[1]{\basicstdstyle{#1}}%

\newcommand{\msprintmean}[1]{{\makebox[\meanlen][r]{\meanstyle{#1}}}}
\newcommand{\msprintstd}[1]{\mssep{\makebox[\stdlen][\msstdalign]{\textsubscript{\stdstyle{#1}}}}}

\newcommand{\setcellformat}[4][l]{
    \renewcommand\msstdalign{#1}%
    \renewcommand\msmfmt{#2}%
    \renewcommand\mssep{#3}%
    \renewcommand\mssfmt{\textsubscript{#4}}%
    \settowidth{\meanlen}{{\msmfmt}}%
    \settowidth{\stdlen}{{\mssfmt}}%
}
% default: \setcellformat[l]{00.00}{\ensuremath{\pm}}{00.00}



\newcommand{\msc}[2][n]{%
    \let\meanstyle\basicmeanstyle%
    \let\stdstyle\basicstdstyle%
    \ifx b#1\let\meanstyle\bfmeanstyle\let\stdstyle\bfstdstyle\fi%
	\setsepchar{,}%
    \reademptyitems%
	\readlist*\theparam{#2}%
    \ignoreemptyitems%
	\readlist*\theneparam{#2}%
    \msprintmean{\theparam[1]}%
    \ifnum \theparamlen=2 
        \ifnum \theneparamlen=2
            \msprintstd{\theparam[2]}%
        \else
            \phantom{\msprintstd{0}}%
        \fi
    \fi
}

\newcommand{\msb}[1]{\msc[b]{#1}}


